A Glimpse Far into the Future: Understanding Long-term Crowd Worker Quality

Microtask crowdsourcing is increasingly critical to the creation of extremely large datasets. As a result, crowd workers spend weeks or months repeating the exact same tasks, making it necessary to understand their behavior over these long periods of time. We utilize three large, longitudinal datasets of nine million annotations collected from Amazon Mechanical Turk to examine claims that workers fatigue or satisfice over these long periods, producing lower quality work. We find that, contrary to these claims, workers are extremely stable in their quality over the entire period. To understand whether workers set their quality based on the task's requirements for acceptance, we then perform an experiment where we vary the required quality for a large crowdsourcing task. Workers did not adjust their quality based on the acceptance threshold: workers who were above the threshold continued working at their usual quality level, and workers below the threshold self-selected themselves out of the task. Capitalizing on this consistency, we demonstrate that it is possible to predict workers' long-term quality using just a glimpse of their quality on the first five tasks.

==> old/tex/abstract_v1.tex <==
Paid crowdsourcing tasks are often simple and repetitive, which fatigues workers over time. We study the temporal effects of this fatigue buildup in paid crowdsourcing across 30 workers during several, repetitive microtasks. On average across all workers during these tasks, the quality of the work produced decreases, which agrees with previous literature on fatigue buildup during simple, repetitive tasks. Additionally, using a collection of six months of task data, we study the fatigue effects in microtasks across thousands of workers. Overall, an emerging trend that paid crowd workers begin to "satisfice" over time - eventually their work converges toward some minimum acceptable quality. 
  
%   To combat both fatigue effects and satisficing, we introduce Burnout, a tool that identifies when a worker is fatigued or is about to start satisficing. Evaluations validate Burnout's accuracy and its ability to be inserted into crowdsourcing pipelines to generate higher quality results.

==> old/tex/conclusion_v1.tex <==
In this paper, we identified satisficing in long-term crowdsourcing and showed that it can have a negative impact on submission quality. For creation-based tasks, such as annotating images with descriptions, we found that the quality decreases greatly over time in both correctness and diversity. On the other hand, we found the satisficing effect to be minimal on verification tasks. Finally, we showed that we could predict satisficing behavior before such behavior begins. 

More generally, we introduce satisficing as a major concern when undertaking long-term crowdsourcing projects. In particular, we challenge the widely-accepted notion that having experienced workers keeps the quality of results high. We introduce a new set of 

==> old/tex/discussion_v1.tex <==
\textbf{Volunteer-based crowdsourcing. }
In this paper, we focus on the long-term worker quality in paid crowdsourcing tasks. In contrast to paid crowdsourcing, volunteer-based crowdsouring platforms, such as citizen science projects~\cite{raddick2013galaxy,rotman2012dynamic,shirk2012public} incentivize workers using intrinsic motivators. While we observe degradation of work quality in paid work, similar analysis is yet to be carried out for volunteer based systems. Do crowd-volunteers take longer to satisfice or show signs of satisficing at all?

\textbf{Preventing satisficing.}
%Refresh your pool
% Prevent satisficing
%   1) Dynamically update the bar of acceptance
%   2)
The most intuitive solution to preventing satisficing is to prevent a worker from completeing further tasks once they start to exhibit signs of satisficing. However, this solution seems a bit unsatisfying for two reasons. First, resetting the worker pool seems a bit unfair to workers who have good intentions but are trying to maximize their efficiency for better pay. Second, rejecting long-term workers does not harness the experience gained by workers to productive use. 

Thus, an alternate solution would be one that prevents satisficing while retaining a worker base. Recall that previous work has tried to do fight fatigue through microdiversions~\cite{dai2015and}, but short breaks do not address nor solve long-term satisficing, as we have demonstrated. One possible mechanic to prevent satisficing could be to dynamically increase the acceptance metrics of a task over time. Consider the image description task we analyzed above. Initially, we might consider a description to be of good quality if it contains at least 5 words. After the worker has completed a certain number of tasks, we might increase the acceptance criteria such that the worker must now submit descriptions that contain at least 7 words. As workers continue to do repetitous tasks, they become proficient at completing them. Increasing the acceptance criteria might incentize the worker to once again improve their ability to perform the task and prevent their quality from decreasing~\cite{gee2004learning}.

Another possible solution would be to give continuous feedback grounded in a worker's output~\cite{dow2012shepherding}. Often times in crowdsourcing workflows, workers complete a task and are never made aware of why their work was accepted or rejected. By receiving external quality measures of their output, worker's might be incentivized to produce high quality work and be informed when their quality begins to dwindle. Future work must also study if workers also become desensitized to incorporating such grounded feedback.

\textbf{Satisficing awareness.}
From a psychological perspective, further investigations must be done to determine whether workers are aware of their diminishing work quality. If they are aware, how do they justify the lower quality and what are the main motivations for doing it?  If they aren't aware, what can be done to either increase awareness or alleviate the onset fatigue?
\rak{Don't say something is interesting. It's up to the reader to determine what is and isn't interesting}

==> old/tex/implications_v1.tex <==
% what to not do: keep 
We find that the quantitative and qualitative drops in submission quality in the region annotation task and QA task demonstrates the problem of long-term worker satisficing for creative tasks. This ubiquitous, long-term decline suggests that previous notions of retaining experienced workers should be reconsidered. Rather than treating workers as constant or improving over time, we must restructure our tasks to accomodate 

==> old/tex/intro_v1.tex <==
Paid crowdsourcing platforms often use \emph{microtasks}, which are atomic, simple tasks that humans perform exceptionally better than their machine counterparts; examples of microtasks include annotating images with semantically correct descriptions or verifying correctness of such descriptions. Microtask oriented markets offer well-defined tasks for workers to easily comprehend and follow, while simultaneously allowing requesters to fully harness the highly parallel and scalable nature of crowdsourcing. However, the microtask formulation, while well-defined and efficient, often results in monotonous sequences of repetitive work.

Although tapping into human cognition provides the ability to complete many crowdsourced tasks, it can also be limiting in both reliability and repeatability. Common knowledge suggests that to circumvent these problems, one would seek a pool of trusted workers that have historically proven to complete high quality work. Thus, to mitigate reliability problems, previous work attempt to find methods to retain these experienced workers in order to obtain high quality and stable results (CITE).  

From other domains, we understand that the performance of human workers is greatly susceptibile to \emph{fatigue}, a temporary drop in cognitive or physical condition gradually onset by a variety of factors, including health, stress, and workload. Fatigue intensifies in boring, repetitive tasks and conditions where workers do not feel to be significantly contributing to a more holistic narrative (CITE). Since the microtask crowdsourcing paradigm bears all these qualities, it develops fatigue rapidly in workers.

As crowdsourcing platforms are usually opt-in, a general belief is that workers can look elsewhere for more interesting tasks whenever they become weary or bored of their current work. However, with the microtask paradigm heavily ingrained, the ability to find new, interesting work becomes difficult. Since a small percentage of full-time crowdsourcing workers complete most of the crowdsourced work, these workers must trade-off searching for interesting work with their pay~\cite{little8020}. 

The majority of crowdworkers primarily work for monetary reasons~\cite{martin2014being}. Therefore, upon finding good work and requesters, it becomes difficult for workers to search for potentially more interesting tasks and give up the already good pay presented. Upon foregoing potential work, workers end up \emph{satisficing}. In economic labor markets, satisficing is defined as a decision-making strategy used to find a situation above some acceptable threshold, usually occurring in cases where optimal solutions are not easily discernible.  In workplace environments, satisficing is defined as the intentional act of meeting the bare minimum requirements for the assigned task.

We propose that satisficing in crowdsourcing is evident, detrimentally affecting the quality of work. The effects of satisficing are often long-term trends with no easily identifiable solutions, as the condition stems from the microtask paradigm as well as the long-term onset of fatigue in workers.

In this paper, we first collected large amounts of data for a creation-based microtask: marking any salient region of an image and writing a description about that region. Over a 9 month span, we collected over 5 million image descriptions from 2,674 workers. We then formulate our research questions about satisficing in crowdworking and define our experimental design with respect to the quality of submitted work over time.

==> old/tex/intro_v2.tex <==
With the rapidly increasing number of recent datasets for computer vision \cite{krishnavisualgenome, lin2014microsoft}, natural language processing, and \akh{INSERT TOPICS + CITATIONS}, studies to better understand crowdsourcing at a large scale must be conducted. In order to fully harness the highly parallel and scalable nature of crowdsourcing, paid crowdsourcing platforms often use \emph{microtasks}, which are atomic, simple tasks that humans perform exceptionally better at than their machine counterparts\cite{bernstein2010soylent,bernstein2011crowds,lasecki2011real,lasecki2012real}. Examples of microtasks include annotating images with semantically correct descriptions or writing coherent, grammatically correct questions tha test a broad understanding of these images~\cite{krishnavisualgenome}. 

Although the microtask formulation offers scalability for requesters and simple tasks for workers, if often results in monotonous sequences of repetitive work~\cite{dai2015and}. Prior work has found that a small minority of workers usually completes a great majority of the work~\cite{little8020}. Therefore, it is imperative that we understand what happens to workers as they repeatedly complete sequences of the same task over a long period of time. Consequently, we pose the question:

\textit{RQ1: Are workers' submissions decreasing in quality over time.}


% Paid crowdsourcing platforms often use \emph{microtasks}, which are atomic, simple tasks that humans perform exceptionally better at than their machine counterparts\cite{bernstein2010soylent,bernstein2011crowds,lasecki2011real,lasecki2012real}; examples of microtasks include annotating images with semantically correct descriptions or writing coherent, grammatically correct questions tha test a broad understanding of these images~\cite{krishnavisualgenome}. Microtask oriented markets offer well-defined tasks for workers to easily comprehend and follow, while simultaneously allowing requesters to fully harness the highly parallel and scalable nature of crowdsourcing. However, the microtask formulation, while well-defined and efficient, often results in monotonous sequences of repetitive work~\cite{dai2015and}.

% Although tapping into human cognition provides the ability to complete many crowdsourced tasks, it can also be limiting in both reliability and repeatability. Common knowledge suggests that to circumvent these problems, one would seek a pool of trusted workers that have historically been proven to complete high quality work. Thus, to mitigate reliability problems, previous work attempt to find methods to retain these experienced workers in order to obtain high quality and stable results~\cite{dai2015and,law2016curiosity}.  


From studies in psychology, we understand that the performance of human workers is greatly susceptibile to \emph{fatigue}, a temporary drop in cognitive or physical condition gradually onset by a variety of factors, including health, stress, and workload~\cite{perelli1980fatigue, boksem2008mental}. Furthermore, we know that fatigue affects workers who engage in sustained work over long periods of time, resulting in performance drops~\cite{krueger1989sustained}. Since the microtask crowdsourcing paradigm often creates monotonous sequences of repetitive work, it should develop fatigue rapidly in workers, posing a potential problem on quality in long-term crowdsourcing.

In this paper, we analyze long-term worker trends over three different real-world, large-scale datasets that were collected for the Visual Genome project~\cite{krishnavisualgenome}: image descriptions, visual question answering, and binary verification for these annotations.  Specifically, we use over $5$ million image descriptions from $2,674$ workers over a $9$ month span and $800$ thousand question-answer pairs from $2,179$ workers over a $3$ month span.  We find that, on average, workers who repeatedly complete microtasks over long periods of time maintain a fairly constant correctness for each task --- contrary to our initial hypothesis that worker's show signs of fatigue over time. Furthermore, we find that workers submit less diverse annotations and are able to complete tasks faster over time.

With these findings of consistency, we were interested in determining whether workers were naturally consistent or whether the task design played an effect. We randomly placed workers into four conditions by varying the acceptance threshold with which we accept or reject work and the transparency in which we give feedback.  Ultimately, we find that workers submit work at the same level of correctness regardless of the acceptance threshold, but often will self-select themselves out of tasks where they believe there is a high risk of rejection. This consistency across different acceptance thresholds demonstrates that workers are naturally consistent.  

If individual workers indeed sustain constant correctness over time, then, intuitively, any subset of a worker's lifetime should be representative of the entire lifetime.  We demonstrate that a simple glimpse of a worker's first few tasks is a strong predictor of long-term performance. A simple average of the first $5$ tasks a worker completes can predict a worker's correctness over his or her entire lifetime with an average error of $3.4\pm3.4\%$.


==> old/tex/intro_v3.tex <==
\rak{Something weird happened to our figure captions. They are no longer bold after I imported the subcaption package to caption subfigures. How do we fix this?}

Micro-task crowdsourcing is rapidly gaining popularity among research communities and businesses as a means
to leverage the highly scalable nature of parallel human computation~\cite{thomee2015new}. Unlike any other service, a crowdsourcing platform is in fact a marketplace subject to human factors that affect its performance, both in terms of speed and quality~\cite{difallahdynamics}. Today, hundreds of thousands of workers on Amazon's Mechanical Turk (AMT) complete tasks that are too challenging for a computer program to solve~\cite{bernstein2010soylent,bernstein2011crowds,lasecki2011real,lasecki2012real}. Crowd workers help generate datasets with millions of annotations by completing tasks over a period of multiple months~\cite{krishnavisualgenome}. As more and more tasks are launched on crowdsourcing platforms, studies must examine the effects of task type, quality control and feedback on crowd workers over long periods of time.

From studies in psychology, we understand that the performance of human workers is greatly susceptibile to \emph{fatigue}, a temporary drop in cognitive or physical condition gradually onset by a variety of factors, including health, stress, and workload~\cite{perelli1980fatigue, boksem2008mental}. Fatigue buildup results in performance drops for people who engage in sustained work over long periods of time~\cite{krueger1989sustained}. Although the microtask formulation offers scalability for requesters and simple tasks for workers, if often results in monotonous sequences of repetitive work~\cite{dai2015and}. Prior work has found that a small minority of workers usually completes a great majority of the work~\cite{little8020}. Therefore, it is imperative that we understand what happens to workers as they repeatedly complete sequences of the same task over a long period of time. Consequently, we pose the question:

\textit{RQ1: How does the quality of workers' submission change over time?}

Since the microtask paradigm in large scale crowdsourcing results in workers repeatedly doing tasks, fatigue buildup can pose a potential problem on the quality of submitted work over time. Do worker's perform worse over time? Do they satisfice to the minimum quality of work required? To study these long term effects on crowd work, we analyze worker trends over three different real-world, large-scale datasets that were collected for the Visual Genome project~\cite{krishnavisualgenome}: image descriptions, visual question answering, and binary verifications.  Specifically, we use over $5$ million image descriptions from $2,674$ workers over a $9$ month span, $800$ thousand question-answer pairs from $2,179$ workers over a $3$ month span, and over $2$ million verifications from $3,913$ workers.

Contrary to our initial hypothesis that workers exhibit signs of fatigue in submission quality over time, we find that workers who repeatedly complete microtasks maintain a consistent correctness for each task, throughout their lifetime \rak{do I need to define lifetime here or is it obvious?}. Furthermore, we find as workers become more experienced on a task, they develop strategies that enable them to complete tasks faster. With these findings of consistency, we are:

\textit{RQ2: Are workers inherently consistent or whether the task design played an effect?}

We randomly placed workers into two different conditions by varying the acceptance \textit{threshold} with which we accept or reject work. If workers in the Visual Genome datasets were consistent only because of their tasks, we expect the workers in the high threshold to perform at a level higher than the ones in the low threshold --- who would satisfice to performing tasks at a quality just above the low threshold. To adequate study the effects of these thresholds, we further divided up the workers into two groups: one where we provided them \textit{transparent} feedback on their quality of work after every single task and another where we simply accepted or reject their work based on the quality. Since most crowdsourcing tasks do not provide explicit feedback after every task, varying the level of transparency allowed us to study satisficing effects in workers who were aware of the acceptance threshold and their current quality of work and ones who did not.

We analyze $676,628$ annotations collected from $1,134$ workers on AMT. we find that poorly performing workers in the high threshold condition would often self-select themselves out of tasks where they believe there is a high risk of rejection. This opting out of workers in the high threshold condition was statistically significant between workers in the two transparent conditions. However, we find that workers submit work at the same level of correctness regardless of the varying acceptance threshold and the transparency condition. Bolstered by the inherent consistency we observe in workers, we ask:

\textit{RQ3: Can we predict a worker's future performance months after they start a working on a microtask?}

If individual workers indeed sustain constant correctness over time, then, intuitively, any subset of a worker's lifetime should be representative of the entire lifetime.  We demonstrate that a simple glimpse of a worker's first few tasks is a strong predictor of long-term performance. A simple average of the quality of work of the first $5$ tasks a worker completes can predict a worker's correctness over their entire lifetime with an average error of $3.4\%$.

Observing that we can identify good consistent workers suggests multiple implications for crowsourcing. We should design crowdsourcing tasks such that we can easily hire good workers and dependably collect high quality annotations~\cite{mitra2015comparing}. Additionally, once we have identified these workers, we can exponentially back off using attention checks to ensure good quality work since we have established that workers quality is unvarying~\cite{liueffective}. Finally, since workers perform at a high quality even if the acceptance threshold is low. By lowering the threshold, we reduce the rejection risk that workers face, increasing worker retention~\cite{difallah2014scaling,law2016curiosity}. In conclusion, we analyze that 

==> old/tex/region-analysis_v1.tex <==
\subsection{Data and Setup}
Using the data collected during the completion of the Visual Genome dataset \cite{krishnavisualgenome}, we use the 5747930 region annotations written by 2,674 workers collected on Amazon Mechanical Turk over 6 months. Each region annotation was collected by having a worker draw a bounding box over a salient part of an image and write a sentence or phrase about that area. The data collection was split into separate Human Intelligence Tasks (HIT), each of which required a worker to create 10 unique region annotations for one image, averaging at least 4 words per annotation. In order to prevent malicious workers, we put simple sanity checks to prevent cheating and tried to ensure diversity with a threshold on the BLEU score \cite{papineni2002bleu} similarity between the different annotations. Furthermore, we sent each region annotation to be verified by three other workers.

\begin{figure}
    \centering
    \includegraphics[width = .45\textwidth]{images/region_HIT.png}
    \caption{An example of the task presented to a worker.}
    \label{fig:region_HIT}
\end{figure}

Figure \ref{fig:sen_worker_dist} shows the distribution of workers on how many HITs they completed over the lifetime of this project. The top 20\% of workers who completed the most HITs did 91.8\% of the total work. Although our distribution is slightly skewed from the standard Pareto 80-20 rule \cite{little8020}, it still demonstrates the fact that a small, but diligent minority does the majority of the work. Therefore, we believe it is necessary to study potential changes of submitted work from this diligent worker group over time.

\begin{figure}
    \centering
    \includegraphics[width = .45\textwidth]{images/sen_worker_dist.eps}
    \caption{The distribution of the number HITs done by each worker}
    \label{fig:sen_worker_dist}
\end{figure}

\subsection{Annotation Correctness Over Time}
The most important and straightforward metric of annotation quality is whether each annotation is correct. To determine correctness, we used a standard verification procedure of majority voting by three different workers. Overall, we notice that workers who repeatedly completed our annotation task severely dropped in quality. When considering those who did at least 100 of our HITs ($n=XXX$), we found that, on average, the percentage of annotations verified to be correct dropped by XXX between the first and last HIT. 
\begin{figure}[t!]
    \centering
    \includegraphics[width =0.45\textwidth]{images/normalized_partitioned_range.eps}
    \caption{Correctness of sentences of workers grouped by how many total HITs they completed.}
    \label{fig:normalized_partitioned_range}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width =0.45\textwidth]{images/normalized_partitioned_first100.eps}
    \caption{Correctness of sentences of workers separated by how correct their region annotations were in their first 100 HITs.}
    \label{fig:normalized_partitioned_first100}
\end{figure}

We were interested in determining whether this substantial drop was ubiquitous among workers, or severly affected a certain group. In Figure \ref{fig:normalized_partitioned_range}, we grouped workers by how many HITs they completed by the end of our data collection and normalized their history to fit between a Start and End mark. We found that the number of HITs had no bearing on the decline between the final difference. Figure \ref{fig:normalized_partitioned_first100} groups these workers by how well they performed on the first 100 HITs, demonstrating that even the best workers are susceptible to this quality decline.

What we find most remarkable is that, for most workers, the trajectory from their start to end is relatively similar. This sigmoid-shaped path from start to end suggests that people have different resistances to fatigue and satisficing. Crowdworkers are known to be risk-averse (CITE), showing the near-perfect start for most workers' lifespans. However, as their work gets continually accepted, we believe the workers are 

\subsection{Loss of Annotation Diversity Over Time}
Since each annotation also contains a phrase or sentence, we examine general syntax trends of the annotations over time.  
\begin{figure}[t!]
    \centering
    \includegraphics[width =0.45\textwidth]{images/ngram_normalized_first100.eps}
    \caption{The degradation of ngram diversity over time. }
    \label{fig:ngram_normalized_first100}
\end{figure}
Figure \ref{fig:ngram_normalized_first100} demonstrates the degradation of diversity in annotation syntax over time. As N-grams are often used in language processing for syntax measurements, we construct a metric of syntax diversity for a set of annotations as follows:
\begin{equation}
    \text{syntax diversity} = \frac{\text{number of unique N-grams}}{\text{number of total N-grams}}.
\end{equation}
If the annotation set contains annotations with different words and ordering, this diversity metric approaches 1, as the amount of unique N-grams will approach the total possible N-grams. If the annotation set contains increasingly similar annotations, many N-grams will be redundant, making this diversity metric approach 0.

Similar to how there exists a global, downward trend when measuring annotation correctness, there also exists a significant degradation of N-gram diversity.

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{images/bothHIT_bbox.pdf}
    \caption{Region annotations submitted by a worker}
    \label{fig:last_bbox}
\end{figure}
% 
% First:  mannequin wearing shorts
% First:  surfboard decorated with photos
% First:  surfboard with photo of Queen Elizabeth II
% First:  mannequin with shorts and towel
% First:  surfboard with black and white photos
% First:  surfboard with photos of young men
% First:  boys are standing on platform and singing
% First:  the wall is blue
% First:  the wall has panelling
% First:  the towel is white
% last:  a light pole behind the plane
% last:  a sign on the runway
% last:  the sign is orange
% last:  the tail is blue
% last:  a yellow strip on the tail
% last:  a star symbol on the tail
% last:  black letters on the airplane
% last:  red letters on the plane
% last:  red letters on the building
% last:  a parking garage behind the plane
% A1YURG2FMHHV7I 1040


% First:  A tall railroad sign 
% First:  A train on a rail
% First:  A train stop station
% First:  Rails on the flat surface
% First:  dry field of lands
% First:  Railroad light signals
% First:  some debris under the rails
% First:  some bushes are extending out
% First:  some sort of electric box
% First:  A legion of trees
% last:  head of a person
% last:  leg of a person
% last:  leg of a person
% last:  feet of a person
% last:  arm of a person
% last:  arm of a person
% last:  hand of a person
% last:  hand of a person
% last:  eye of a person
% last:  eye of a person
% A1U3H2XORT4V75 3832

% First:  slice of pizza with toppings
% First:  Chunk of tomato on a slice of pizza
% First:  cheesy slice of pizza
% First:  crust on a slice of pizza
% First:  slice of pizza with tomatoes and spinach
% First:  spinach topping on a slicce of pizza
% First:  Pizza cut into 8 slices
% First:  burnt piece of crust on slice of pizza
% First:  slice of pizza with tomatoes and spinach
% First:  cheesy slice of pizza
% last:  picket fence is white
% last:  elephant in front of elephant
% last:  elephant in front of elephant
% last:  elephant walking behind elephant
% last:  white tusk on elephant
% last:  white tusk on elephant
% last:  white tusk on elephant
% last:  trees behind three elephants
% last:  ear on large elephant
% last:  ear on large elephant
% A2CK8S4CH1HPBE 1887

% First:  the man wearing a wetsuit is kite boarding 
% First:  the kite boarder is controlling the kite with the cables and harness
% First:  another kite boarder with a green, white and blue kite is in the distance
% First:  hills are seen in the distant horizon
% First:  the white caps mean it is a windy day and perfect for kite boarders
% First:  a buoy in the harbor mark maritime channels and hazards
% First:  it's a clear day with perfect visibility to keep a look out for a great white shark
% First:  kiteboard foot straps are needed to keep the kite boarder feet in place
% First:  blue skies and no clouds mean for a clear day and no rain
% First:  the kite boarders wet suit should keep him warm and dry
% last:  seagull hovering over a hotdog stand
% last:  girl in an orange coat sitting on a wall
% last:  man in a blue jacket eating a hotdog
% last:  seagulls eating on the street
% last:  blue and yellow canopy umbrella on the cart
% last:  man in blue jacket wearing glasses
% last:  man eating hotdog wearing ear muffs
% last:  lady vendor in a brown jacket
% last:  stack of sodas on the hotdog cart
% last:  black tire on the hotdog cart
% ACPWJRT77OKF4 1420




\subsection{Convergence Between Different Workers}
Although workers seem to individually lose diversity in their annotations, what global trends emerge between different workers?

\begin{figure}[t!]
    \centering
    \includegraphics[width =0.45\textwidth]{images/similarity.eps}
    \caption{Similarity matrices between the annotations of workers who did over 1000 HITs in their first HIT and their last HIT.}
    \label{fig:similarity1000}
\end{figure}

One aspect we measure is the similarity of the annotations submitted by workers over time. To measure the similarity between two sets of annotations, we use a basic cosine distance metric on N-grams \cite{damashek1995gauging}. We first build a sparse word vector represenation of the counts in each annotation set and then compute the cosine distance. This metric outputs a value closer to 1 as the sets become increasingly identical and outputs values closer to 0 as the annotation sets become increasingly distinct. Figure \ref{fig:similarity1000} shows the increase in similarity between workers' annotations as they continually do the annotation task. 

\begin{figure*}[t!]
  \centering
  \includegraphics[width=\textwidth]{images/word_distribution.eps}
  \caption{Word Distribution at the first HIT (top row) and last HIT (bottom row) across workers who have done at least 1000 HITs. Each column corresponds to the word distribution a specific word index in the annotation. For example, the second column corresponds to the distribution of an annotation's second word.}
  \label{fig:word_distribution}
\end{figure*}


==> old/tex/related_v1.tex <==
Our work was inspired by psychology, decision making, and workplace management literature that focus on identifying the major factors that affect the quality of work produced. Specifically, we look at the effects of fatigue and satisficing in the workplace. We then look at how these problems transfer to the crowdsourcing domain. Finally, we explore the efficacy of existing crowdworker retention techniques for addressing these problems to establish a gap in these techniques.

\textbf{Fatigue.}
Repeatedly completing the same task generally induces boredom in workers. The United States Air Force found that both the cognitive performance and physical conditions of its airmen continually deteriorated during the course of long, mandatory shifts~\cite{perelli1980fatigue}. Unlike these mandatory duties, crowdsourcing is generally opt-in for workers - they do not need to continually keep working, as they have the option to break whenever they feel tired or bored. However, previous work has shown that people cannot accurately gauge how long they need to rest after working continuously, resulting in an incomplete recoveries and drops in task performance after breaks~\cite{hennfng1989microbreak}. Additionally, other studies have shown that the primary indicator of fatigue is linked to the motivation of the workers, rather than the total time worked~\cite{beckers2004working}. 

Although crowdsourcing has shown to have the potential to be intrinsicially motivating~\cite{von2006games}, the microtask paradigm found in the majority of the tasks favors a structure that is efficient for workers rather than being interesting for them.


\textbf{Satisficing.}
In his paper, Herbert Simon introduces the concept of satisficing as an approach taken when the complexity or uncertainty of the global outcomes of a decision make determining the optimal choice impossible~\cite{simon1972theories}. A satisficing decision can be equated to an approximate, local search of the optimum, rather than sieving through all possible choices. To further narrow this search, satisificers set an aspiration level, a minimum acceptance criterion grounded in the reality of their situations, and choose any option that meets this aspiration level. 

Crowdworkers avoid the most difficult parts of a task whenever possible~\cite{mason2010financial}.

% An example of a maximizing decision would be determining the next chess move during the endgame - the sample space is sufficiently small enough to determine a global optimum. Alternatively, a decision that entails satisficing would be the entire strategy one adopts to checkmate the opponent - with the nearly infinite combinations to do so, it becomes impossible for the human mind to determine what is the best solution.

\textbf{Improving Crowdsourcing Quality.}
External checks such as verifiable gold standards, requiring explanations, and majority voting are standard practice for reducing bad answers and quality control~\cite{kittur2008crowdsourcing,callison2009fast}. Other methods directly estimate worker quality to improve these external checks~\cite{ipeirotis2010quality,whitehill2009whose}. By giving external feedback or having crowdworkers internally reflect on their prior work also has been shown to yield better results~\cite{dow2012shepherding}. Previous work directly targets the monotony of crowdsourcing, showing that by framing the task as more meaningful to workers (for example as a charitable cause), one obtains higher quality results~\cite{chandler2013breaking}. Other work has identified that responders to surveys often satisfice~\cite{krosnick1991response}, reducing the quality of data. Disguised checks in the instructions~\cite{oppenheimer2009instructional} or rate-limiting the presentation of the questions~\cite{kapelner2010preventing} greatly improves the detection and prevention of satisficing during crowdsourced surveys. However, this framing study only had workers do each task once and did not observe long-term trends.

\textbf{Worker Retention.}
As mentioned previously, much work has been done on retaining a pool of good, experienced workers that continually submit high-quality work. Some techniques for such retainment include piquing workers' curiosity, <INSERT MORE>~\cite{law2016curiosity}. Interestingly, previous research in this worker retention area identifies fatigue as a potential source of error and uses carefully timed micro-diversions to alleviate short-term fatigue~\cite{dai2015and}.  However, simply retaining a worker pool does not adequately address satisficing issues that may arise as this pool repeatedly completes microtasks over longer periods of time.

==> old/tex/related_v2.tex <==
Our work was inspired by psychology, decision making, and workplace management literature that focus on identifying the major factors that affect the quality of work produced. Specifically, we look at the effects of fatigue and satisficing in the workplace. We then look at how these problems transfer to the crowdsourcing domain. Finally, we explore the efficacy of existing crowd worker quality improvement techniques.

\textbf{Fatigue.}
Repeatedly completing the same task over a sustained period of time will induce fatigue. Fatigue has shown to increase reaction time, decrease production rate, and is linked to a rise in poor decision-making in workers~\cite{krueger1989sustained, wyatt1937fatigue}.  The United States Air Force found that both the cognitive performance and physical conditions of its airmen continually deteriorated during the course of long, mandatory shifts~\cite{perelli1980fatigue}. However, unlike these mandatory, sustained shifts,  crowdsourcing is generally opt-in for workers - there always exists the option for workers to break whenever they feel tired or bored. Nonetheless, previous work has shown that people cannot accurately gauge how long they need to rest after working continuously, resulting in incomplete recoveries and drops in task performance after breaks~\cite{hennfng1989microbreak}. Additionally, other studies have shown that the primary indicator of fatigue is linked to the motivation of the workers, rather than the total time worked~\cite{beckers2004working}. Although crowdsourcing has shown to have the potential to be intrinsicially motivating~\cite{von2006games}, the microtask paradigm found in the majority of crowdsourcing tasks favors a structure that is efficient for workers rather than being interesting for them.

\textit{RQ1: What are the effects of fatigue on workers who repeatedly complete the same crowdsourcing task?}

Ultimately, we find that previous literature arrives at the following hypothesis:

\textit{H1: Fatigue causes workers to submit lower quality work over time.}

\textbf{Worker Retention and Crowdsourcing Over Time.}
As mentioned previously, much work has been done on retaining a pool of good, experienced workers that continually submit high-quality work. Some techniques for such retainment include piquing workers' curiosity~\cite{law2016curiosity} and pricing schemes for microtasks~\cite{difallah2014scaling}. Interestingly, previous research in this worker retention area identifies fatigue as a potential source of error and uses carefully timed micro-diversions to alleviate short-term fatigue~\cite{dai2015and}.  

However, simply building techniques to retain a worker pool does not adequately study how these retained workers perform over time. Previous research has shown that once crowdsourced ideas are found to be valuable, the original ideator often generates less diverse ideas~\cite{bayus2013crowdsourcing}.

In his paper, Herbert Simon introduces the concept of satisficing as an approach taken when the complexity or uncertainty of the global outcomes of a decision make determining the optimal choice impossible~\cite{simon1972theories}. A satisficing decision can be equated to an approximate, local search of the optimum, rather than sieving through all possible choices. To further narrow this search, satisificers set an aspiration level, a minimum acceptance criterion grounded in the reality of their situations, and choose any option that meets this aspiration level. An example of satisficing in crowdsourcing occurs when workers avoid the most difficult parts of a task whenever possible~\cite{mason2010financial}.

\textit{RQ2: What }


\textbf{Improving Crowdsourcing Quality.}
External checks such as verifiable gold standards, requiring explanations, and majority voting are standard practice for reducing bad answers and quality control~\cite{kittur2008crowdsourcing,callison2009fast}. Other methods directly estimate worker quality to improve these external checks~\cite{ipeirotis2010quality,whitehill2009whose}. By giving external feedback or having crowdworkers internally reflect on their prior work also has been shown to yield better results~\cite{dow2012shepherding}. Previous work directly targets the monotony of crowdsourcing, showing that by framing the task as more meaningful to workers (for example as a charitable cause), one obtains higher quality results~\cite{chandler2013breaking}. Other work has identified that responders to surveys often satisfice~\cite{krosnick1991response}, reducing the quality of data. Disguised checks in the instructions~\cite{oppenheimer2009instructional} or rate-limiting the presentation of the questions~\cite{kapelner2010preventing} greatly improves the detection and prevention of satisficing during crowdsourced surveys. However, this framing study only had workers do each task once and did not observe long-term trends.



==> old/tex/rq.tex <==
\fl{Data}
\sl{Image Descriptions}
Using the data collected during the completion of the Visual Genome dataset \cite{krishnavisualgenome}, we use the 5747930 region annotations written by 2,674 workers collected on Amazon Mechanical Turk over 6 months. Each region annotation was collected by having a worker draw a bounding box over a salient part of an image and write a sentence or phrase about that area. The data collection was split into separate Human Intelligence Tasks (HIT), each of which required a worker to create 10 unique region annotations averaging at least 4 words per annotation. In order to prevent malicious workers, we put simple sanity checks to prevent cheating and tried to ensure diversity with a threshold on the BLEU score \cite{papineni2002bleu} similarity between the different annotations. Furthermore, we sent each region annotation to be verified by three other workers.

\begin{figure}
    \centering
    \includegraphics[width = .45\textwidth]{images/region_HIT.png}
    \caption{An example of the task presented to a worker.}
    \label{fig:region_HIT}
\end{figure}

Figure \ref{fig:sen_worker_dist} shows the distribution of workers on how many HITs they completed over the lifetime of this project. The top 20\% of workers who completed the most HITs did 91.8\% of the total work. Although our distribution is slightly skewed from the standard Pareto 80-20 rule \cite{little8020}, it still demonstrates the fact that a small, but diligent minority does the majority of the work. Therefore, we believe it is necessary to study potential changes of submitted work from this diligent worker group over time.

\begin{figure}
    \centering
    \includegraphics[width = .45\textwidth]{images/sen_worker_dist.eps}
    \caption{The distribution of the number HITs done by each worker}
    \label{fig:sen_worker_dist}
\end{figure}

\subsection{Does the quality of submitted work change over time?} 

From previous literature, we expect that crowd workers should exhibit significant fatigue and satisficing related effects as they repeatedly finish our task. 


% Introduce the 3 research questions:

% 1) As workers complete more and more of the same task, what happens to the quality of their submitted work over long periods of time?

% 2) If there is an effect on quality, what types of tasks are most susceptible to this effect? 

% 3) 

==> old/tex/trends__Michael_Bernstein_s_conflicted_copy_2016-08-01_.tex <==
In this section, we perform an analysis of worker behavior over time on three large-scale data collection efforts on AMT. We describe the three datasets and the tasks used to gather the data, all drawn from the following machine learning data labeling tasks: image descriptions, question answering, and verification. We then examine common trends, such as worker accuracy and annotation diversity over time. We use these results to answer whether workers are suffering from fatigue or other decreases in effectiveness over time. %Finally, we use these observations to infer answers to the research questions proposed earlier in the paper about the effects of  fatigue and task familiarity. 

\first{Data}
\akh{new} Each of the following three tasks were priced such that workers could earn $\$6$ per hour and were available to workers with a $95\%$ approval rating and who live in the United States. For the studies in this paper, workers were tracked by their AMT worker id's. Before we begin our analysis, we first describe the $3$ datasets that we inspect~\footnote{The tasks and interfaces used to collect the data are described in detail in the Visual Genome paper~\cite{krishnavisualgenome}. Each microtask was allocated $2.5$ hours but could be completed in within $5$ minutes, ensuring that workers didn't feel any time pressure.}.

\akh{R1 wants the time we gave each worker and description we put on AMT. not sure if relevant or how to insert (AC echoed this)}\rak{Already addressed this below.}

\second{Image descriptions.}
An image description is a phrase or sentence associated with a certain part of an image. To complete this task, a worker looks at a complex scene image, clicks and drags to select an area of the image, and then describes it using a short textual phrase (e.g., ``The dog is jumping to catch the frisbee''). Each image description task requires a worker to create $5-10$ unique descriptions for one randomly selected image, averaging at least $5$ words per description. Workers were asked to keep the descriptions factual and avoid submitting any speculative phrases or sentences. Over $9$ months, $5,380,263$ image descriptions were collected from $2,674$ workers on AMT. \msb{average time to completion per task? (for each of these)}

\second{Question answers.}
Each question answering task asks a worker to write $7$ questions and their corresponding answers for $2$ different, randomly selected images. Workers were instructed to begin each sentence with one of the following questions: who, what, when, where, why and how~\cite{kuhn2013political}. Furthermore, to ensure diversity of question types, workers were asked to write a minimum of $4$ of these question types. Workers were also instructed to be concise and unambiguous to avoid wordy and speculative questions. In total, over $830,625$ questions were generated by $2,179$ workers over $3$ months.

\second{Binary verifications.}
Verification tasks were quality control tasks: given an image and a question-answer pair, workers were asked if the question was relevant to the image and if the answer accurately responded to the question. The majority decision of three workers was used to determine the accuracy of each question answering pair. Over $2.6$ million votes were cast by $3,913$ workers over $3$ months. For each verification task, a worker had to vote on $50$ randomly ordered question answering pairs.

\second{Overall.} 
Figure~\ref{fig:dist_workers} shows the distribution of how many tasks workers completed over the span of the data collection period. The top $20\%$ of workers who completed the most tasks did $91.8\%$, $90.9\%$, and $88.9\%$ of the total work in each of the three datasets respectively. These distributions are similar to the standard Pareto $80$-$20$ rule~\cite{little8020}, clearly demonstrating that a small, but persistent minority of workers completes an extremely large number of similar tasks. To demonstrate that workers may work for very extended periods of time on the same task, we noticed that for each of the three tasks types, the top $1\%$ of workers did $5.5$, $0.7$, and $1.0$ thousand tasks \msb{awkward, just list the number} on average. If each worker took $4$ minutes for image descriptions and question answering tasks and $2$ minutes for verification tasks \msb{not a sentence}. The estimated average work time equates to $15$, $2.1$, and $1.4$ days of continuous work \msb{clarify this is non-stop, and also give the number in terms of 8hr work days}. \akh{new - do you think this adequately answers the question ``how is this study extended/generalized to longer periods of time''. If not, maybe we should iterate in the section ``workers are consistent over long periods'' below?} \rak{I think the next line is sufficient.} \msb{seems like you also want to add the long-long-long term caveat to limitations. like, we don't (yet) have data over years. But I think it's fair to note that many crowdsourced data collection tasks don't actually take years --- the big ones are more like ours, large amounts of work that last a few weeks to months. However, we should note that there are others (e.g., Jon Brelig) that have been going on for years.} Additionally, we found that workers, on average, spread the time they worked on these tasks across $10$ weeks for the image description task. By the final week of the data collection, about $10\%$ of the workers remained working on the tasks, suggesting that our study captures the entire lifetime of many of these workers. \msb{something like, ```However, some crowdsourcing tasks (e.g., Jon Brelig) have persisted longer than this. We focus on these days-to-months crowd worker relationships, leaving analysis of multi-year relationships to future work.''}


\begin{table}
    \centering
    \begin{tabular}{l | r r r}
        & Annotations & Tasks & Workers \\ \hline
         \rule{0pt}{2ex}Descriptions & $\num[group-separator={,}]{5380263}$& $\num[group-separator={,}]{605443}$ & $\num[group-separator={,}]{2674}$ \\ 
         Question Answering & $\num[group-separator={,}]{830625}$ & $\num[group-separator={,}]{54587}$ & $\num[group-separator={,}]{2179}$ \\
         Verification & $\num[group-separator={,}]{2689350}$ & $\num[group-separator={,}]{53787}$  & $\num[group-separator={,}]{3913}$ \\ 
         
    \end{tabular}
    \caption{The number of workers, tasks, and annotations collected for image descriptions, question answering, and verifications}
    \label{tab:dataset}
\end{table}

We focus our attention in this paper on workers who completed at least $100$ tasks during the span of the data collection. The completion time for $100$ tasks is approximately $6.7$ hours for image description and question answering tasks and $3.3$ hours for verification tasks. We find that $657$, $128$, and $177$ workers completed $100$ of the image descriptions, QA, and verification tasks respectively. The median worker in each task type completed $349$, $220$, and $181$ tasks, which translates to $23.2$, $14.6$, and $6.0$ hours of continuous work.  These workers also produced $94.5\%$, $70.5\%,$ and $66.3\%$ of each of the total amount of the annotations. These worker pools are relatively unique: there are $61$ shared workers between image descriptions and QA, $69$ shared workers between image descriptions and verifications, and $42$ shared workers between question answering and verifications. \rak{bonus: add how many workers were in all 3. Complete that ven diagram!}

\akh{Demographics stats}

After all tasks were completed, we reached out to these $815$ unique workers who had worked on at least $100$ tasks and asked them to complete a survey. After collecting $280$ responses, we found the gender distribution to be $73.3\%$ female, $24.3\%$ male, and $0.4\%$ other. Furthermore, we found that workers with ages $30$-$49$ were the majority at $54.3\%$ of the long-term worker population. Ages $18$-$29$, $50$-$64$, and $65+$ respectively comprised $19.2\%$, $23.0\%$ and $3.4\%$ of the long-term worker population. Compared to the distributions in previously gathered demographics on AMT~\cite{pew2016, difallah2014scaling,ross2010crowdworkers}, the distribution of long-term workers is older and comprised of more females. However, when we consider all workers who contributed to these datasets, the distribution closely aligns with these other previously gathered ones~\cite{krishnavisualgenome}. Previous work has found that the female and older worker demographic groups on average have lower wages than their counterparts~\cite{pew2016}. Thus, we hypothesize that these worker groups' inclination to work on stable, long-term projects may preclude them from briefer, but higher paying opportunities.  

\akh{I feel as though reviewers will want an explanation. This may make VG look bad though}

\begin{figure}[t]
    \centering
    \includegraphics[height=1.2in]{images/gender_pie}
    \includegraphics[height=1.2in]{images/age_bars.pdf}
    \caption{Self reported gender (left) and age distribution (right) of 280 workers who completed at least $100$ of the image description, question answer, or binary verification tasks. \akh{New figure}}
    \label{fig:correctness}
\end{figure}

\first{Workers are consistent over long periods}
We analyzed worker accuracy and annotation diversity over the entire period of time that they worked on these tasks. Because workers performed different numbers of tasks, we normalize time data to percentages of their total \textit{lifetime}, e.g., when they were at the halfway point in terms of the total number of tasks completed. 

\second{Annotation accuracy.} A straightforward metric of quality is the percentage of microtasks that are correct. To determine accuracy for an image description or question answering task, we used a majority vote over a separate verification task. However, measuring the quality of the verification dataset is more difficult. Since the ground truth of verification tasks is unknown at such a large scale, we need a metric to estimate the accuracy of each verification decision. We believe that comparing a worker's vote against the majority decision is a good approximation of accuracy. To test this, we randomly sampled a set of $15,000$ descriptions and question answers to be sent back through the verification pipeline $6$ months after the initial dataset was collected, and found a $99.3\%$ similarity between the majority decision of this new verification process with the original decision reported in the dataset~\cite{krishnavisualgenome}. The result of this test indicates that the majority decision is repeatable and a good standard to compare against. 

We find that workers change very little over time (Figures~\ref{fig:correctness} and~\ref{fig:qa_individuals}). When considering those who did at least 100 image description tasks, people on average started at $97.9\pm12.1\%$  accuracy and ended at $96.6\pm9.1\%$, averaging an absolute change of $3.3\pm5.6\%$. Workers who did at least $100$ question answering tasks started with an average of $88.4\pm6.3\%$ and ended at $87.5\pm6.0\%$, resulting in an absolute change of $3.1\pm3.3\%$. For the verification task, workers agreed with the majority on average $88.1\pm3.6\%$ at the start and $89.0\pm4.0\%$ at the end, resulting in an absolute change of $3.1\pm3.4\%$. Inspecting the lifetime curves (Figures~\ref{fig:correctness} and~\ref{fig:qa_individuals}), there is also little evidence of a learning curve at the beginning of the lifetime, suggesting that workers were familiar with these task styles.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/correctness.pdf}
    \caption{The average accuracy over the lifetime of each worker who completed over $100$ tasks in each of the three datasets. The top row shows accuracy for image descriptions, the middle row shows accuracy for question answering, and the bottom row shows accuracy for the verification dataset. }
    \label{fig:correctness}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/qa_individuals.pdf}
    \caption{A selection of individual workers' accuracy over time during the question answering task. Each worker remains relatively constant throughout his or her entire lifetime. }
    \label{fig:qa_individuals}
\end{figure}

\second{Annotation diversity.}
Accuracy captures clearly correct or incorrect outcomes, but how about subtler signals of effort level?
Since each image description or question answer task produces multiple phrases or questions, we examine the linguistic similarity of these phrases and questions over time. As N-grams have often been used in language processing for gauging similarity between documents~\cite{damashek1995gauging}, we construct a metric of syntax diversity for a set of annotations as follows:
\begin{equation}
    \text{diversity} = \frac{\text{number of unique N-grams}}{\text{number of total N-grams}}.
\end{equation}
As the annotation set increasingly contains different words and ordering of words, this diversity metric approaches 1 because the amount of unique N-grams will approach the total possible N-grams. Conversely, if the annotation set contains increasingly similar annotations, many N-grams will be redundant, making this diversity metric approach 0. To account for workers reusing similar sentence structure in consecutive tasks, we track the number of unique N-grams versus total N-grams in sequential pairs of tasks.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/bigram.pdf}
    \caption{On average, workers who repeatedly completed the image description (top row) or question answering (bottom row) tasks gave descriptions or questions with increasingly similar syntactic structures.}
    \label{fig:bigram}
\end{figure}

The percentage of unique bigrams decreases slightly over time (Figure~\ref{fig:bigram}). For workers in the image description task, the percent of unique bigrams decreases from $82.4\%$ to $78.4\%$ between the start and end of a worker's lifetime. Since there are $4.2$ bigrams on average per phrase, a worker writes approximately $42$ total bigrams per task. Thus, a decrease in $4.0\%$ results in a loss of $1.7$ unique bigrams per task. For workers who completed the question answering tasks, the percent of unique bigrams decreases from $60.7\%$ to $54.0\%$. As there are on average $3.4$ bigrams per question, this $6.7\%$ decrease would cost a loss of $3.2$ distinct bigrams per task. Ultimately, these results show that over the course of a worker's lifetime, only a small fraction of diversity is lost, as less than a sentence or question's contribution of bigrams is lost.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/bothHIT_bbox.pdf}
    \caption{\akh{New Figure and changed description}Image descriptions written by a satisficing worker on a task completed near the start of their lifetime (left) and their last completed task (right). Despite the images being visually similar, the phrases submitted in the last task are much less diverse than the ones submitted in the earlier task.}
    \label{fig:both_bbox}
\end{figure}

Although the majority of the worker pool stays relatively constant during their lifetime, we noticed that there were a few workers who, although writing factually correct image descriptions and questions, have a sharper decrease and an extremely lower N-gram diversity by the end of their lifetime. This behavior describes a completely ``satisficing'' worker, as they repeatedly write the same types of sentences or questions that generalize to almost every image. Figure~\ref{fig:both_bbox} demonstrates how the phrase diversity decreases between the first and last submitted image description task for these satisficing workers. To determine the percentage of total workers who are satisficing workers, we set a threshold as the difference between the maximum diversity and mean diversity, and find the percent of workers who drop below the mean by this threshold is about $7\%$ and $2\%$ of workers in the image description and question answering datasets respectively. 

\second{Annotation speed.}
We recorded the time it takes on average for workers to complete a single verification. We removed $2.4\%$ of the datapoints deemed as outliers from this computation, as workers will infrequently take longer times during a break or while reading the instructions. \akh{defined outlier computation}We defined outliers for each task of 50 verifications as times that outside 3 standard deviations of the mean time for those 50 verifications. Overall, Figure~\ref{fig:qa_ver_time} demonstrates that workers indeed get faster over time. Initially, workers start off taking $4.5$ seconds per verification task, but end up averaging under $3.4$ seconds per task, resulting in an approximate $25\%$ speedup. Although no time data was recorded for either the image descriptions or question answering tasks, we believe that they would also exhibit similar speedups over time due to practice effects~\cite{newell1981mechanisms} and similarities in the the correctness and diversity metrics.


%We recorded the time it takes on average for workers to complete a single verification. We removed $3.74\%$ of the datapoints deemed as outliers from this computation, as workers will infrequently take longer times during a break or while reading the instructions. \akh{defined outlier computation}We defined outliers for each task of 50 verifications as times that outside 2 standard deviations of the mean time for those 50 verifications \msb{The typical nmber in statistics is three standard deviations}. Overall, Figure~\ref{fig:qa_ver_time} demonstrates that workers indeed get faster over time. Initially, workers start off taking $3.7$ seconds per verification task, but end up averaging under $2.5$ seconds per task, resulting in a $32\%$ speedup. Although no time data was recorded for either the image descriptions or question answering tasks, we believe that they would also exhibit similar speedups over time due to practice effects~\cite{newell1981mechanisms} and similarities in the the correctness and diversity metrics.

\first{Discussion}

\second{No significant fatigue effects.} Workers do not appear to suffer from long-term fatigue effects. With an insignificant average accuracy drop of on average $1.5\%$ for workers across their lifetime, we find that workers demonstrate little change in their submission quality. Instead of suffering from fatigue, workers have the option to opt-out or break whenever they feel tired~\cite{dai2015and}. Furthermore, this finding seems to agree with previous literature that performance drops are not as affected by cumulative fatigue as physically straining conditions such as disrupted circadian rhythm~\cite{perelli1980fatigue}.

\second{Accuracy is constant within task, but varies across tasks.} We attribute the similarity between the average accuracy of the question answering and verification tasks to being part of the same crowdsourcing pipeline.  Additionally, we notice the average accuracy for image descriptions is noticeably higher than the average accuracy for either the question answering or verification datasets. We believe this discrepancy stems from the question answering task's instructions to write four distinct types of \emph{W} questions, as some question types such as ``why'' or ``when'' are often ambiguous for many images. Furthermore, we also attribute the disparity between unique bigram percentage for the image description and question answering tasks to the question answering task's instructions that asked workers to begin each question with one of the $7$ question types.

\second{Experience Translates to Efficiency.} Workers retain constant accuracy, and slightly reduce the complexity of their writing style. Combined, these findings suggest that workers find a general strategy that leads to acceptance and stick with it. Studies of practice effects suggest that a practiced strategy helps to increase worker throughput according to a power law~\cite{newell1981mechanisms}. This power law shape is clearly evident in the average verification speed, confirming that practice plays a crucial role in the worker speedup. 

\second{Overall Findings.} From an analysis of the three datasets, we found that fatigue effects are not significantly visible and that severe satisficing behavior only affects a very small proportion of workers. On average, workers maintain a similar quality of work over time, but also get more efficient as they gain experience with the task.


==> old/tex/verification-analysis_V1.tex <==
\subsection{Data and Setup}
With the use of verification as a measure for quality decrease, we must also consider that verifiers' work might also degrade over time. Each verification task consists of 50 annotations in which each worker can mark correct or not correct. An annotation is marked correct if the phrase truthfully describes what is contained in the bounding box. However, if the bounding box does not fully encapsulate or is over the wrong part of the image, we deem the annotation incorrect. In total, we collected 7278850 completed verification tasks from 1628 workers. (THIS ISNT 3X REGION ANNOTATIONS, HOW TO DEAL WITH IT)

\subsection{Verification Correctness Over Time}
Since ground truth of the verification task is unknown at such a large scale, we believe that a good approximation of correctness entails comparing a worker's vote against the majority decision.

\begin{figure}
    \centering
    \includegraphics[width =0.45\textwidth]{images/qa_ver_agreement.pdf}
    \caption{Agreement with the majority decreases over the course of a worker's lifespan in verification tasks}
    \label{fig:qa_ver_agreement}
\end{figure}

Figure \ref{fig:qa_ver_agreement} displays the how verifiers agree less as they complete more HITs. 


